$\epsilon$-Kernel Coresets for Stochastic Points

With the dramatic growth in the number of application domains that generate probabilistic, noisy and uncertain data, there has been an increasing interest in designing algorithms for geometric or combinatorial optimization problems over such data. In this paper, we initiate the study of constructing $\epsilon$-kernel coresets for uncertain points. We consider uncertainty in the existential model where each point's location is fixed but only occurs with a certain probability, and the locational model where each point has a probability distribution describing its location. An $\epsilon$-kernel coreset approximates the width of a point set in any direction. We consider approximating the expected width (an \expkernel), as well as the probability distribution on the width (an \probkernel) for any direction. We show that there exists a set of $O(1/\epsilon^{(d-1)/2})$ deterministic points which approximate the expected width under the existential and locational models, and we provide efficient algorithms for constructing such coresets. We show, however, it is not always possible to find a subset of the original uncertain points which provides such an approximation. However, if the existential probability of each point is lower bounded by a constant, an exp-kernel\ (or an fpow-kernel) is still possible. We also construct an quant-kernel coreset in linear time. Finally, combining with known techniques, we show a few applications to approximating the extent of uncertain functions, maintaining extent measures for stochastic moving points and some shape fitting problems under uncertainty.

==> beta.tex <==
\subsection{$\beta$-Assumption}

We discuss a specific assumption in this section, under which special structure is guaranteed to exist with high probability.  Conditioning on this structure makes certain coreset results possible and other algorithms easier.

In particular, we assume that each possible location realizes a point with a probability at least $\beta$, where $\beta >0$ is some fixed constant (e.g. is not $O(1/n)$).  We refer to this as \emph{the $\beta$-assumption}.
So in the existential model each $p_v \geq \beta$ and in the locational model each $p_{s,v} \geq \beta$.
This should seem quite reasonable in practice since often if a location is part of the data set, it has likely been measured above some threshold of probability.  Moreover in the locational model, it is often assumed that each uncertain point takes on one of $k$ possible locations, each with probability $1/k$, and $k$ is a small constant.


\begin{lemma}
\label{lm:specialpt}
Given the $\beta$-assumption, there exists a point $c^\star \in \R^d$ that is in the convex hull of the realized uncertain points with probability at least $1-1/n$.
\end{lemma}
\begin{proof}
A point $c^\star$ is in the convex hull of a point set $X$, if in \emph{every} direction $u$ there is a halfspace $H_u$ which has $c^\star$ on its boundary and contains at least one point of $P$.
Let $\calH$ be the set of all halfspaces.  An $\eps$-net of $(X,\calH)$ is a subset $Y \subset X$ such that each halfspace $H \in \calH$ which contains at least $\eps |X|$ points of $X$ contains at least $1$ point of $Y$.

We show that a point $c^\star$ is in the convex hull of the points $P$ realized from $\calP$ with high probability.  For existential points $c^\star$ is the centerpoint of all potential points $\calP$ and in the location model, consider the location $s$ of each uncertain point $\calP$ with the highest probability, and let $c^\star$ be the centerpoint of those $n$ points.
%The centerpoint $c$ of a set of $n$ points has the property that \emph{every} halfspace which contains $c$ 
%also contains at least $n/(d+1)$ points from $P$.
Recall that a point $c$ is a centerpoint for a set $X$ of $n$ points if every halfspace containing $c$ also contains at least $n/(d+1)$ from $X$.
Thus if $P$ is an $(1/(d+1))$-net of $\calP$, then for every direction $u$, the associated halfspace $H_u$ must contain at least one point $P$, and thus $c^\star$ is in the convex hull.  Thus it remains to show that with high probability $P$ is an $(1/(d+1))$-net of $\calP$.

It is known that a random sample of size $O((d/\eps) \log (1/\eps \delta))$ is an $\eps$-net for halfspaces in $\R^d$ with probability at least $1-\delta$.  Thus for some absolute constant $C$ a sample of size $C d(d+1) \log (n (d+1))$ is a $(1/(d+1))$-net with probability at least $1-1/n$.  Since each point $v \in \calP$ is realized in $P$ with probability $\beta > C d (d+1) \log (n(d+1)) / n$, then the point set realized $P$ is an $(1/(d+1))$-net and thus contains $c^\star$ in its convex hull, with probability at least $1-1/n$.
\end{proof}



==> coreset.tex <==
\section{Minimum $j$-Flat-Center}
\label{sec:coreset}
\eat{
\begin{definition}
\label{def:jflat}
Given a set $\calP$ of $n$ uncertainty points (in either locational or existential model) in $\R^d$. Given a $j$-flat $F\in \calF$ ($0\leq j\leq d-1$), where $\calF$ is the family of all $j$-flats in $\R^d$. We define the distance between $\calP$ and $F$ as follows:
$$
\dist(\calP,F)=\Exp_{P\sim \calP}[\max_{p\in P}\dist(p,F)].
$$
Minimum $j$-flat-center problem is to find a $j$-flat which minimizes the value $\dist(\calP,F)$.
\end{definition}

\begin{definition}
\label{def:jkproj}
Given a set $P$ of $n$ points in $\R^d$. Define a weight function $w:P\rightarrow \R^*$. For sme $0\leq j\leq d-1$ and $k\geq 1$, let $\calF$ be the family of shapes with each shape being a union of $k$ $j$-subspaces in $\R^d$. For a point $p\in \R^d$ and a shape $F\in \calF$, define $\dist(p,F)=\min_{q\in F}\dist(p,q)$. Let $\cost(P,F)=\sum_{s_i\in P}w_i\dist(s_i,F)$. A weighted $(j,k)$-projective clustering problem is to find a shape $F\in \calF$ which minimizes the value $\cost(P,F)$.
\end{definition}
}

In this section, we consider a more general shape fitting problem, the minimum $j$-flat-center problem in the stochastic models. Our main technique is to construct a coreset of constant size such that for any $j$-flat $F\in \calF$, we can use the coreset to obtain a ($1\pm \e$)-estimation for $\dist(\calP,F)$. Then since the coreset is of constant size, we have a polynomial system of constant size to compute the optimum in constant time.

Let $A=\sum_{1\leq i\leq n}p_i$ be the total probability. We discuss two different cases. If $A<\e$, we reduce the problem to a weighted ($j,1$)-projective clustering problem, which has been studied in~\cite{varadarajan2012sensitivity}. If $A\geq\e$, the construction of the coreset can be divided into two parts, one estimating the contribution of high probability points by an \exprkernel, and the other one estimating the contribution of the rest low probability points by reducing to a weighted ($j,1$)-projective clustering problem. The definition of the weighted ($j,1$)-projective clustering problem is as follows.

\begin{definition}
\label{def:jkproj}
Given a set $P$ of $n$ points in $\R^d$, define a weight function $w:P\rightarrow \R^*$. For some $0\leq j\leq d-1$ and $k\geq 1$, let $\calF$ be the family of shapes with each shape being a union of $k$ $j$-subspaces in $\R^d$. For a point $p\in \R^d$ and a shape $F\in \calF$, define $\dist(p,F)=\min_{q\in F}\dist(p,q)$. Let $\cost(P,F)=\sum_{s_i\in P}w_i\dist(s_i,F)$. A weighted $(j,k)$-projective clustering problem is to find a shape $F\in \calF$ which minimizes the value $\cost(P,F)$.
\end{definition}

\subsection{Case 1: $A<\e$}

In the first case, we show that the minimum $j$-flat-center problem can be reduced to a weighted ($j,1$)-projective clustering problem, and construct a coreset of constant size. We need the following lemmas.

\begin{lemma}
\label{lm:sjflattoj1}
If $A<\e$, for any $j$-flat $F\in \R^d$, we have $\sum_{s_i\in \calP}p_i\cdot\dist(s_i,F)\in (1\pm \e)\cdot\dist(\calP,F)$.
\end{lemma}

\begin{proof}
For a $j$-flat $F\in \R^d$, w.l.o.g., we assume that $\dist(s_i,F)$ is non-decreasing in $i$. Thus, we have
$$
\dist(\calP,F)=\sum_{i\in [n]}p_i\cdot \dist(s_i,F)\cdot\prod_{j>i}(1-p_j)
$$
Since $A<\e$, for any $i\in [n]$, we have that $1-\e\leq 1-\sum_{j\in [n]}p_i\leq \prod_{j>i}(1-p_j)\leq 1$. So we prove the lemma.
\end{proof}

By Lemma~\ref{lm:sjflattoj1}, we reduce the original problem to a weighted $(j,1)$-projective clustering problem, where each point $s_i\in \calP$ has weight $p_i$. The next step is to find an $\e$-coreset $S$ for this problem, which is defined as follows:
\begin{definition}
Given a (weighted) instance $P\subset \R^d$ of a shape fitting problem $(\R^d,\calF,\dist)$ with weight function $p:P\rightarrow \R^+$, an $\e$-coreset of $P$ is a (weighted) set $S\subseteq P$, together with a weight function $w:S\rightarrow \R^+$, such that that for any shape $F\in \calF$, we have
$$ \sum_{s_i\in S}w_i \cdot \dist(s_i,F)\in (1\pm \e)\sum_{s_i\in P}p_i\cdot \dist(s_i,F).
$$
The size of the weighted coreset $S$ is defined to be $|S|$.
\end{definition}
We first introduce a definition called 'sensitivity'. Then we show that we can bound the size of the $\e$-coreset $S$ by the total sensitivity.

\begin{definition} (Sensitivity of a shape fitting instance~\cite{langberg2010}). Given an instance $P\subset \R^d$ of a shape fitting problem $(\R^d,\calF,\dist)$, the sensitivity of a point $p$ in $P$ is $\sigma_P(p):=\inf\{\beta\geq 0\mid \dist(p,F)\leq \beta \cdot \dist(P,F), \forall F\in \calF\}$. The total sensitivity of $P$ is defined by $\mathfrak{G}_{P}=\sum_{p\in P}\sigma_P(p)$.
\end{definition}

\begin{lemma}
\label{lm:sentocore} (\cite{FL11})
Given any $n$-point instance $P\subset \R^d$ of a shape fitting problem $(\R^d,\calF,\dist)$, and any $\e\in (0,1]$, there exists an $\e$-coreset for $P$ of size $O((\frac{\mathfrak{G}_n}{\e})^2 \dim(P))$. Here, $\mathfrak{G}_n$ denotes the total sensitivity of the $n$ points, and $\dim(P)$ denotes the dimension of the shape fitting instance $P$. In the $(j,k)$-projective clustering problem, the dimension $\dim(P)$ of any instance $P$ is $O(jdk)$.
\end{lemma}

We still need to show that the total sensitivity of all $j$-flats is bounded by a constant by the following lemmas.

\begin{lemma}
\label{lm:totalsen}
Consider the weighted $(j,1)$-projective clustering problem where $\calF$ is the set of all $j$-flats in $\R^d$. The total sensitivity of any weighted $n$-point set is $O(j^{1.5})$.
\end{lemma}

The proof of Lemma~\ref{lm:totalsen} is similar to that of Theorem 18 in~\cite{varadarajan2012sensitivity} except that we consider the weighted version. The details can be found in Appendix~\ref{app:coreset}.
As in~\cite{varadarajan2012sensitivity}, our method for bounding the total sensitivity directly can be translated into a polynomial time algorithm for computing $\e$-coresets. Combining Lemma~\ref{lm:sentocore} an~\ref{lm:totalsen}, we conclude the main lemma in this subsection.

\begin{lemma}
\label{lm:psmall}
Given an instance $\calP$ of $n$ uncertain points in $\R^d$, if the total probability $\sum_i p_i<\e$, there is an $\e$-coreset of size $O(j^{3.5}d\e^{-2})$ for the minimum $j$-flat-center problem. Moreover, we have a polynomial time algorithm to compute the $\e$-coreset.
\end{lemma}

\eat{
\topic{Algorithm.}
\begin{enumerate}
\item Compute the optimal shape $F^*$. (It suffices to use a constant approximately optimal shape.) Compute $\calP'$ which is the projection of $\calP$ onto $F^*$.
\item Based on $\calP'$, compute a bound on the sensitivity of each point. By Lemma~\ref{lm:dimreduction}, we translate these sensitivities into a bound for $\sigma_{\calP}(s_i)$ for each $s_i\in \calP$.
\item Sample points from $\calP$ with probabilities proportional to $\sigma_{\calP}(s_i)$ to obtain a coreset.
\end{enumerate}
Therefore, the key point is how to find a constant approximately optimal shape $F^*$. By Theorem 4.4 in~\cite{deshpande2011algorithms}, the authors show that there is an algorithm to compute a constant approximately optimal shape $F^*$ with high probability via convex programming.
}

\subsection{Case 2: $A\geq \e$}

Note that if $F$ is a $j$-flat, the function $\dist(x,F)^2$ has a linerization. We have the following lemma to bound the dimension of the linearization.

\begin{lemma} (\cite{feldman2013turning})
\label{lm:dimofl}
Suppose $F$ is a $j$-flat in $\R^d$, the function $\dist(x,F)^2$ ($x\in \R^d$) has a linerization. Let $D$ be the dimension of the linearization. If $j=0$, we have $D=d+1$. If $j=1$, we have $D=O(d^2)$. Otherwise, for $2\leq j\leq d-1$, we have $D=O(j^2d^3)$.
\end{lemma}

Suppose $\calP$ is an instance of $n$ uncertain points in $\R^d$. For each $j$-flat $F\in \R^d$, let $h_F(x)=\dist(x,F)^2$ ($x\in \R^d$), which admits a linearization of dimension $O(j^2d^3)$ by Lemma~\ref{lm:dimofl}. Now, proceeding as for the minimum enclosing ball problem in Section~\ref{subsec:shapefitting}, we map each point $s\in \calP$ into an $O(j^2d^3)$ dimensional point $s'$ and map each $j$-flat $F\in \R^d$ into an $O(j^2d^3)$ dimensional direction $u$, such that $\dist(s,F)=\innerprod{s'}{u}^{1/2}$. By this mapping, we translate our goal into finding a direction $u\in \R^{O(j^2d^3)}$, which minimizes the value $\Exp_{P\sim \calP}[\max_{x\in P}\innerprod{u}{x}^{1/2}]$.

Using the same method of constructing \probkernel\ in Section~\ref{subsec:2}, we construct a convex hull $\calH=\cap_u H_u$. Recall that $H_u$ denotes the halfplane defined by the sweep line $\ell_u$ (orthogonal to the normal vector $u$)
and $\bH_u$ denotes its complement. The difference is that we stop the movement of $\ell_u$ at the first point such that $\Prob[\calP\cap \bH_u)]\geq \e'$, where $\e'$ is a constant determined later. By Lemma~\ref{lm:lambdasumhigh}, we construct a convex set $\calK$, which is the intersection of $O(1/\epsilon^{O(j^2d^3)})$ halfspaces and satisfies that $(1-\e)\calK\subseteq \calH\subseteq \calK$. Let $\bcalK=\calP\setminus \calK$. Let $\e'=\epsilon^{O(j^2d^3)}$, which makes sure that $\Prob[\bcalK]\leq \e$.
\footnote{This is because that $\Prob[\bcalK]$ is upper bounded by the multiplication of $\e'$ and the number of halfspaces of $\calK$.}

We construct an $(\e'\cdot \e(1-\e),2)$-\textsc{fpow-kernel} $S_1$ for points in $\calK$. We show that we can estimate $\Exp_{P\sim \calK}[\max_{x\in P}\innerprod{u}{x}^{1/2}]$ by $S_1$. For the rest points in $\bcalK$, we show that the contribution for the objective function $\Exp_{P\sim \calP}[\max_{x\in P}\innerprod{u}{x}^{1/2}]$ is almost linear and can be reduced to a weighted $(j,1)$-projective clustering problem as in Case 1. We first prove the following lemma.

\begin{lemma}
\label{lm:exprkernel}
For any direction $u\in \calP^{\polar}$, we have the following property.
$$
\Exp_{P\sim S_1}[\max_{x\in P}\innerprod{u}{x}^{1/2}]+\sum_{s_i\in \bcalK} p_i \cdot \innerprod{u}{s_i}^{1/2} \in (1\pm 4\e)\Exp_{P\sim \calP}[\max_{x\in P}\innerprod{u}{x}^{1/2}].
$$
\end{lemma}

\begin{proof}
Let $E$ be the event that no point is present in $\bcalK$. We first rewrite $\Exp_{P\sim \calP}[\max_{x\in P}\innerprod{u}{x}^{1/2}]$ as follows:
\begin{align*}
&\Exp_{P\sim \calP}[\max_{x\in P}\innerprod{u}{x}^{1/2}]=\Prob[E]\cdot \Exp_{P\sim \calP}[\max_{x\in P}\innerprod{u}{x}^{1/2}\mid E]+\Prob[\overline{E}]\cdot\Exp_{P\sim \calP}[\max_{x\in P}\innerprod{u}{x}^{1/2}\mid \overline{E}] \\
=& \Prob[E]\cdot \Exp_{P\sim \calK}[\max_{x\in P}\innerprod{u}{x}^{1/2}]+\Prob[\overline{E}]\cdot\Exp_{P\sim \calP}[\max_{x\in P}\innerprod{u}{x}^{1/2}\mid \overline{E}]
\end{align*}
By the definition of $(\e,2)$-\textsc{fpow-kernel}, for any direction $u\in \calP^{\polar}$, we have that
$$
\Exp_{P\sim S_1}[\max_{x\in P}\innerprod{u}{x}^{1/2}]\in (1\pm \e'\cdot \e(1-\e))\Exp_{P\sim \calK}[\max_{x\in P}\innerprod{u}{x}^{1/2}].
$$
By the construction of $\calK$, we have that $(1-\e)\calK\subseteq \calH$ and $\Prob[\calP\cap (1-\e)\bH_u]\geq \e'$. Thus, we obtain that
$$
\Exp_{P\sim \calP}[\max_{x\in P}\innerprod{u}{x}^{1/2}]\geq \e'(1-\e)\max_{x\in \calK}\innerprod{u}{x}^{1/2}\geq \e'(1-\e) \Exp_{P\sim \calK}[\max_{x\in P}\innerprod{u}{x}^{1/2}].
$$
So we conclude that
\begin{equation}
\label{eq:1}
\begin{split}
&\Prob[E]\cdot \Exp_{P\sim \calK}[\max_{x\in P}\innerprod{u}{x}^{1/2}]- \e\Exp_{P\sim \calP}[\max_{x\in P}\innerprod{u}{x}^{1/2}]\leq \Exp_{P\sim S_1}[\max_{x\in P}\innerprod{u}{x}^{1/2}] \\
\leq &(1+ 2\e)\Prob[E]\cdot \Exp_{P\sim \calK}[\max_{x\in P}\innerprod{u}{x}^{1/2}]+ \e\Exp_{P\sim \calP}[\max_{x\in P}\innerprod{u}{x}^{1/2}],
\end{split}
\end{equation}
since $1-\e\leq \Prob[E]\leq 1$.

For event $\overline{E}$, without loss of generality, we assume that the $n$ points $s_1,\ldots,s_n$ in $\calP$ are sorted in nondecreasing order according to the inner product $\innerprod{u}{s_i}$. Assume that $s_{i_1},\ldots,s_{i_l}$ ($i_1<i_2<\ldots<i_l$) are points in $\bcalK$. Let $E_j$ be the event that point $s_{i_j}$ is present and all points $s_{i_k}$ are not present for $k>j$. Denote $E^+_j$ to be the event that point $s_{i_j}$ is the farthest point according to direction $u$, i.e., $\innerprod{u}{s_{i_j}}$ is the maximum. Note that event $E^+_j$ implies event $E_j$. Let $E^-_j$ be the event that $E_j$ happens while $E^+_j$ does not happen. We have that
\begin{align*}
& \Prob[\overline{E}]\cdot\Exp_{P\sim \calP}[\max_{x\in P}\innerprod{u}{x}^{1/2}\mid \overline{E}]=\sum_{j\in [l]}p_{i_j}\cdot\bigl(\prod_{j+1\leq k\leq l}(1-p_{i_k})\bigr)\cdot\Exp_{P\sim \calP}[\max_{x\in P}\innerprod{u}{x}^{1/2}\mid \overline{E_j}] \\
= & \sum_{j\in [l]}p_{i_j}\cdot\bigl(\prod_{j+1\leq k\leq l}(1-p_{i_k})\bigr)\cdot \bigl(\Prob[E^+_j]\cdot\innerprod{u}{s_{i_j}}^{1/2}+\Prob[E^-_j]\cdot \Exp_{P\sim \calP}[\max_{x\in P}\innerprod{u}{x}^{1/2}\mid E^-_j]\bigr).
\end{align*}
By the above equality, on one hand, we have that
\begin{equation}
\label{eq:2}
\Prob[\overline{E}]\cdot\Exp_{P\sim \calP}[\max_{x\in P}\innerprod{u}{x}^{1/2}\mid \overline{E}]\geq (1-\e)\sum_{j\in [l]}p_{i_j}\cdot \innerprod{u}{s_{i_j}}^{1/2}.
\end{equation}
On the other hand, the following inequality also holds.
\begin{equation}
\label{eq:3}
\begin{split}
&\Prob[\overline{E}]\cdot\Exp_{P\sim \calP}[\max_{x\in P}\innerprod{u}{x}^{1/2}\mid \overline{E}]\leq \sum_{j\in [l]}p_{i_j}\bigl( \Prob[E^+_j]\cdot \innerprod{u}{s_{i_j}}^{1/2}+\Prob[E^-_j]\cdot \Exp_{P\sim \calP}[\max_{x\in P}\innerprod{u}{x}^{1/2}\mid E^-_j]\bigr)\\
\leq & \sum_{j\in [l]}p_{i_j}\cdot \innerprod{u}{s_{i_j}}^{1/2}+ \sum_{j\in [l]}p_{i_j}\cdot \Exp_{P\sim \calP}[\max_{x\in P}\innerprod{u}{x}^{1/2}]\leq  \sum_{j\in [l]}p_{i_j}\cdot \innerprod{u}{s_{i_j}}^{1/2}+ \e\cdot \Exp_{P\sim \calP}[\max_{x\in P}\innerprod{u}{x}^{1/2}]
\end{split}
\end{equation}
The first inequality holds since that $\Prob[E^-_j]\cdot \Exp_{P\sim \calP}[\max_{x\in P}\innerprod{u}{x}^{1/2}\mid E^-_j]\leq \Exp_{P\sim \calP}[\max_{x\in P}\innerprod{u}{x}^{1/2}]$. Combining Inequalities \eqref{eq:1}, \eqref{eq:2} and \eqref{eq:3}, we prove the lemma.
\end{proof}

\eat{
Note that our construction of coreset $S_1$ is under the subset constraint. Thus we can map $S_1$ to original points and obtain the following lemma.

\begin{lemma}
\label{lm:originexprkernel}
For any $j$-flat in $\R^d$, we have the following property.
$$
\Exp_{P\sim S_1}[\max_{x\in P}\dist(x,F)]+\sum_{s_i\in \calP\cap \overline{\calH}} p_i \cdot \dist(s_i,F) \in (1\pm 4\e)\Exp_{P\sim \calP}[\max_{x\in P}\dist(x,F)].
$$
\end{lemma}
}

By Lemma~\ref{lm:psmall}, we construct an $\e$-coreset $S_2$ to estimate $\sum_{s_i\in \bcalK} p_i \cdot \dist(s_i,F)$. Then $S=S_1\cup S_2$ is a nice coreset of constant size, which satisfies the following property:
$$
\Exp_{P\sim S_1}[\max_{x\in P}\innerprod{u}{x}^{1/2}]+\sum_{s_i\in S_2} w_i \cdot \innerprod{u}{s_i}^{1/2} \in (1+ O(\e))\Exp_{P\sim \calP}[\max_{x\in P}\innerprod{u}{x}^{1/2}].
$$
Here $w_i$ is the weight of $s_i$ in $S_2$. By Theorem~\ref{thm:exprconstruction}, we have that the size of $S_1$ is $O(\e^{-O(j^4d^6)})$. By Lemma~\ref{lm:psmall}, we have that the size of $S_2$ can be bounded by $O(j^{3.5}d\e^{-2})$. So we conclude the following lemma.
\begin{lemma}
\label{lm:plarge}
Given an instance $\calP$ of $n$ uncertain points in the existential model, if the total probability $A\geq\e$, there is an $\e$-coreset of size $O(\e^{-O(j^4d^6)}+j^{3.5}d\e^{-2})$ for the minimum $j$-flat-center problem.
\end{lemma}

Combining Lemma~\ref{lm:psmall} and Lemma~\ref{lm:plarge}, we can obtain the following theorem.

\begin{theorem}
\label{thm:j1exist}
Given an instance $\calP$ of $n$ uncertain points in the existential model, there is an $\e$-coreset of size $O(\e^{-O(j^4d^6)}+j^{3.5}d\e^{-2})$ for the minimum $j$-flat-center problem. Moreover, we have a polynomial time algorithm to compute the $\e$-coreset.
\end{theorem}

\topic{Locational Uncertainty Model} Note that in the locational uncertainty model, we only need to consider Case 2. We use the same construction as in the existential model. Let $p_i=\sum_{j}p_{ji}$. Similarly, we make a linearization for the function $\dist(x,F)^2$, where $x\in\R^d$ and $F$ is a $j$-flat in $\R^d$. Using this linearization, we also map $\calP$ into $O(j^2d^3)$ dimensional points. For the $j$th node and a set $P$ of points, we denote $p_j(P)=\sum_{s_i\in P}p_{ji}$ to be the total probability that the $j$th node locates inside $P$.

By the condition $\Prob[\bcalK]\leq \e$, we have that $\Prob[E]=1- \prod_{j\in [m]}(1-p_j(\bcalK))\leq 1-(1-\e)=\e $, where event $E$ represents that there exists a point present in $\bcalK$. So we can regard those points outside $\calK$ independent. On the other hand, for any direction $u$, since $\Prob[\calP\cap (1-\e)\overline{\calH}_u]\geq \e'$, we have that $\Prob[E_u]=1-\prod_{j\in [m]}(1-p_j(\calP\cap (1-\e)\bH_u))\geq 1-(1-\frac{\e'}{m})^m\geq \e'/2$, where event $E_u$ represents that there exists a point present in $\calP\cap (1-\e)\bH_u$. Moreover, note that an $(\e'\cdot \e(1-\e),2)$-\textsc{fpow-kernel} also exists in the locational uncertainty model. So Lemma~\ref{lm:exprkernel} still holds. Then by Lemma~\ref{lm:plarge}, we can construct a coreset of constant size.

\begin{theorem}
\label{thm:j1location}
Given an instance $\calP$ of $n$ uncertain points in the locational uncertainty model, there is an $\e$-coreset of size $O(\e^{-O(j^4d^6)}+j^{3.5}d\e^{-2})$ for the minimum $j$-flat-center problem. Moreover, we have a polynomial time algorithm to compute the $\e$-coreset.
\end{theorem}

\topic{Remark:} We can generalize the above result by considering other distance functions. In fact, we can solve a class of distance functions $\mathsf{dist}(\cdot,\cdot)=\|\cdot\|^z$ for $z\geq 1$. Note that the Euclidean distance function is a special case when $z=1$.

